RADE: Reference-Assisted Dialogue Evaluation for Open-Domain Dialogue

Evaluating open-domain dialogue systems is challenging for reasons such as the one-to-many problem, i.e., many appropriate responses other than just the golden response. As of now, automatic evaluation methods need better consistency with humans, while reliable human evaluation can be time- and cost-intensive. To this end, we propose the Reference-Assisted Dialogue Evaluation (RADE) approach under the multi-task learning framework, which leverages the pre-created utterance as reference other than the gold response to relief the one-to-many problem. Specifically, RADE explicitly compares reference and the candidate response to predict their overall scores. Moreover, an auxiliary response generation task enhances prediction via a shared encoder. To support RADE, we extend three datasets with additional rated responses other than just a golden response by human annotation. Experiments on our three datasets and two existing benchmarks demonstrate the effectiveness of our method, where Pearson, Spearman, and Kendall correlations with human evaluation outperform state-of-the-art baselines.

==> sections/07-discussion.tex <==
\section{Discussion}\label{sec:dis}


\emph{Reliability of human annotation metrics.}
To verify that our human annotation metrics listed in Table~\ref{metrics} are reliable, we invite 20 experts and 80 users and count their approval rates for these metrics.
The results are listed in Figure~\ref{fig:user_study}. We can see that more than 80\% experts and 87.5\% random users think that the \emph{Relevance}, \emph{Engagingness}, and \emph{Fluency} are reliable and agree these metrics are necessary abilities an open-domain dialogue agent should equal. 
The results indicate that these general metrics can be used to evaluate various open-domain dialogue tasks. 
Moreover, the approval rates of three task-specific criteria (i.e., \emph{Understandability}, \emph{Emotional} and \emph{Personality}) exceed 80\% for both experts and users, which indicates these metrics are reliable to evaluate the specific open-domain dialogue tasks.

\begin{figure}
\centering
% \vspace{-3em}
    \includegraphics[width=0.5\textwidth]{figures/evaluation2.pdf}
    % \vspace{-3em}
    \caption{Ruslut of two-role user study. }
    \label{fig:user_study}
    % \vspace{-1em}
\end{figure}


\emph{How to generalizing RADE to other dialogue tasks?}\todo{}
Our experiments show that the proposed RADE model achieves comparable or better performance than state-of-the-art baselines in all benchmarks after the pre-train.
For simplicity, it can be used for other open-domain dialogue tasks out of the box.
Moreover, we find it highly effective to fine-tune the model on task-specific data at the expense of its ability in other domains.


\emph{How to combine the scores from different metrics into the overall score?}\todo{}
We also attempt to sum all scores weighted by approval rate besides taking the averages, which has less impact on the final result.
Some work, e.g., USR~\citep{mehri2020usr}, USL~\citep{usl} explore more configurable methods by training a regression to learn the weights between the different indicators.
However, the approval rate of different metrics is almost the same.



==> tables/combination.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[!t]
\renewcommand\arraystretch{1.1} 
\centering
\caption{Criteria employed to assess models in our human evaluation with high approval rates.
Relevance, human-like and fluency are general view while the rest depend on specific task.
The lastest two column is the result of two-role user study, including the approval rate of experts and random users. 
We also show other low-agreement criteria in Appendix.
}
\begin{tabular}{c|r p{5.5cm} c c}
\hline
 & Criteria      & Explanation &\begin{tabular}[p{1cm}]{@{}c@{}}Approval Rate \\ of Experts\end{tabular}  & \begin{tabular}[p{1cm}]{@{}c@{}}Approval Rate \\ of Users\end{tabular} \\
\hline
% \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}general \\ ability\end{tabular}}  
\multirow{3}{*}{\rotatebox{90}{General ability\quad}}  
& \textit{Relevance:}       &  \textit{Whether the response matches the dialogue context semantically. } & 0.89   & 0.88  \\
 & \textit{Human-like: }      &  \textit{Whether the response is engaging or interesting rather than rigid template.}  & 0.85   & 0.78    \\
 & \textit{Fluency:}          & \textit{Whether the response is fluent and natural throughout the conversation.}  & 0.77 & 0.83 
 \\ \hline
% \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}specific \\ ability\end{tabular}} 
\multirow{3}{*}{\rotatebox{90}{specific ability\quad} } 
& \textit{Informative:}  &  \textit{Is there any external knowledge contained in the response.}  & 0.82 & 0.80  \\
& \textit{Emotional-aware:}  & \textit{whether the agent capture the emotion  of user and support empathic support.} & 0.87 & 0.72  \\
& \textit{Personality-aware:} & \textit{whether the response conforms to given dentity and personality.} & 0.77 & 0.87\\ 
\hline
\end{tabular}

\label{combination}
\end{table*}
